Learnable Uncertainty under Laplace Approximations

Laplace approximations are classic, computationally lightweight means for constructing Bayesian neural networks (BNNs). As in other approximate BNNs, one cannot necessarily expect the induced predictive uncertainty to be calibrated. Here we develop a formalism to explicitly "train" the uncertainty in a decoupled way to the prediction itself. To this end, we introduce uncertainty units for Laplace-approximated networks: Hidden units associated with a particular weight structure that can be added to any pre-trained, point-estimated network. Due to their weights, these units are inactive -- they do not affect the predictions. But their presence changes the geometry (in particular the Hessian) of the loss landscape, thereby affecting the network's uncertainty estimates under a Laplace approximation. We show that such units can be trained via an uncertainty-aware objective, improving standard Laplace approximations' performance in various uncertainty quantification tasks.

==> contents/93_training_setups.tex <==
%!TEX root = ../appendix.tex

In all our experiments, training and predictions are done using a consumer workstation PC with eight CPU cores and a GPU with $11$GB memory.

\subsection{UCI regression}

For each baseline method, the hyperparameters (learning rate, weight decay, and likelihood precision\footnote{We do not optimize the likelihood precision of DE since it already learns heteroscedastic models.}) are found via Bayesian optimization \citep{nogueira2014bayesianopt}, maximizing the validation log-likelihood. Training is done via Adam optimizer \citet{kingma2014adam} for $40$ epochs. The dropout rate of MCD is set to $0.05$, following \citet{gal2016dropout}. KFL is used to construct the Laplace approximation.


\subsection{Image classification}

We use the LeNet architecture for MNIST experiment, trained using Adam for $100$ epochs with an initial learning rate of $0.001$ which was then divided by $50$ at epochs $75$, and $90$. Meanwhile, an eight-layer CNN architecture is used in the CIFAR-10 and CIFAR-100 experiments. In these experiments, we trained the networks for $200$ epochs using SGD with momentum $0.9$ and initial learning rate $0.01$, which was then divided by $10$ at epochs $100$ and $150$. For all networks, we use the SELU activation function without batch normalization. For MCD, we use dropout at every hidden layer with a rate of $0.2$, following \citep{kendall2017uncertainties}. For DE, we train $5$ networks to form the ensemble. The weight decays are set to the same commonly-used value $5\mathrm{e}{-3}$ and $5\mathrm{e}{-4}$ for MNIST and CIFARs, respectively. We use the commonly used data augmentations, such as random cropping and flipping.

We trained LULA for a single epoch (since for each dataset, we have a large amount of training points) with learning rate $0.01$. For each dataset, the number of the additional last-layer units $m_L$ is obtained via a grid search over the set $\{ 32, 64, 128, 256, 512 \} =: M_L$, minimizing the absolute distance to the optimal MMC, i.e. $1$ and $1/k$ for the in- and out-distribution validation set, respectively:
%
\begin{equation*}
    m_L = \argmin_{m \in M_L} \abs{1 - \text{MMC}_\text{in}(m)} + \abs{1/k - \text{MMC}_\text{out}(m)} \, ,
\end{equation*}
%
where $\text{MMC}_\text{in}$ and $\text{MMC}_\text{out}$ are the validation in- and out-distribution MMC of the Laplace-approximated, trained-LULA, respectively.

